Large Reasoning Models Are (Not Yet) Multilingual Latent Reasoners

Large reasoning models (LRMs) achieve strong performance on mathematical reasoning tasks, often attributed to their capability to generate explicit chain-of-thought (CoT) explanations. However, recent work shows that LRMs often arrive at the correct answer before completing these textual reasoning steps, indicating the presence of latent reasoning -- internal, non-verbal computation encoded in hidden states. While this phenomenon has been explored in English, its multilingual behavior remains largely unknown. In this paper, we conduct a systematic investigation of multilingual latent reasoning in LRMs across 11 languages. Using a truncation-based strategy, we examine how the correct answer emerges as the model is given only partial reasoning traces, allowing us to measure stepwise latent prediction formation. Our results reveal clear evidence of multilingual latent reasoning, though unevenly: strong in resource-rich languages, weaker in low-resource ones, and broadly less observable on harder benchmarks. To understand whether these differences reflect distinct internal mechanisms, we further perform representational analyses. Despite surface-level disparities, we find that the internal evolution of predictions is highly consistent across languages and broadly aligns with English -- a pattern suggesting an English-centered latent reasoning pathway.

==> latex/perturbation.tex <==
\section{Perturbation Details}\seclabel{perturbation_details}

We used the two perturbation methods in \secref{edit_method} to probe memorization versus (latent) reasoning.
Both methods operate \emph{only} on the subset of MGSM instances that the model answers correctly under \textbf{pass@10} when the truncation ratio is \textbf{0\%} (i.e., with an empty \texttt{<think>\texttt{</think>}} block).
For each selected instance, we produce two edited variants: \textbf{NumEdit} (meaning-altering) and \textbf{Paraphrase} (meaning-preserving).

\subsection{NumEdit}\seclabel{numedit}

NumEdit creates a minimally changed but \emph{meaning-altering} counterfactual by perturbing exactly \emph{one} number in the question.
The expected behavior differs depending on whether the model relies on memorization or reasoning:
a memorization-driven model may continue to output the original answer, whereas a reasoning-driven model should adapt its answer to the changed quantity.

\paragraph{Numeric span detection.}
We identify candidate numbers using a conservative regular expression that matches standalone numeric tokens (including optional negative sign and decimal part), while avoiding matches that are embedded in words or common formats that are likely to break semantics:
\begin{itemize}
    \item \textbf{Exclude years:} numbers matching \texttt{19xx} or \texttt{20xx} are skipped.
    \item \textbf{Exclude ordinals:} tokens followed by \texttt{st/nd/rd/th} are skipped.
    \item \textbf{Exclude fractions:} occurrences adjacent to \texttt{/} (e.g., \texttt{1/2}) are skipped.
\end{itemize}

\paragraph{Perturbation rule.}
Among the remaining candidates, we perturb \emph{exactly one} numeric span with a small additive change:
\begin{itemize}
    \item If the token is an integer:
    \begin{itemize}
        \item For $\{0,1,2\}$, add $+1$.
        \item Otherwise add a small $\Delta\in\{1,2\}$ (seeded randomness).
    \end{itemize}
    \item If the token is a float, add a small fixed delta depending on magnitude:
    $+0.1$ for $|x|<1$, $+0.5$ for $|x|<10$, otherwise $+1.0$.
\end{itemize}

\subsection{Paraphrase}

Paraphrase produces a meaning-preserving rewrite intended to reduce lexical overlap with the original prompt while keeping the problem logically equivalent.
Unlike NumEdit, the gold answer remains the same.
Thus, high performance on paraphrased questions supports generalization beyond surface-form memorization.

\paragraph{LLM-based Question Paraphrasing.}
We leverage \texttt{Gemini-2.5-Flash} to paraphrase each question.
We have the following constraints in the prompt to ensure that the paraphrased question is equivalent to the original one:
\begin{enumerate}
    \item[-] Preserve all numbers exactly.
    \item[-] Preserve all LaTeX math segments (anything inside \texttt{\$...\$}) exactly as-is.
    \item[-] Maintain logical equivalence and ask for the same final quantity.
    \item[-] Do not add/remove constraints, entities, or units.
\end{enumerate}
To prevent crosslingual drift, we additionally specify that the paraphrase must be written in the same language as the input question.
The prompt template is shown in Figure~\ref{fig:paraphrase_prompt}.

\paragraph{Automatic validation.}
Each paraphrase is validated before acceptance: the multiset of numeric tokens in the paraphrase must match the original. If not, the same prompt will be applied again until the paraphrased question is valid.

\subsection{Perturbation Solvability}

To verify that the generated counterfactual questions remain \emph{solvable} and do not introduce unintended artifacts, we conduct an auxiliary evaluation using a strong commercial model again (\texttt{Gemini-2.5-Flash}).
This analysis serves as a sanity check that the perturbations preserve mathematical well-formedness while modifying surface form or numerical content as intended.

\paragraph{Setup.}
For each selected MGSM problem, we query the model on three inputs: the original question, its NumEdit variant, and its Paraphrase variant (for each input, we only query once).
The model is instructed to optionally generate intermediate steps but to output a single final answer in a strict, parseable format (see prompt in Figure~\ref{fig:gemini_solvability_prompt}).
We then compare Gemini's predictions across variants.
Specifically, we report:
(i) \textbf{Orig Acc}, Gemini's accuracy on the original question;
(ii) \textbf{NumEdit Match}, the proportion of NumEdit predictions identical to the original prediction (lower is better, as the gold answer is expected to be changed); and
(iii) \textbf{Paraphrase Match}, the proportion of Paraphrase predictions identical to the original prediction (higher is better, as the gold answer is expected to be preserved).

\paragraph{Results and Discussion.}
Table~\ref{tab:gemini_counterfactuals} shows that Gemini achieves consistently high accuracy on the original questions across models and languages, indicating that the selected problem subset is reliably solvable.
For NumEdit, the matching ratio remains low (typically below 10\%), confirming that the numerical perturbations effectively alter the solution and are not trivially ignored.
In contrast, Paraphrase variants exhibit very high matching ratios (often above 95\%), demonstrating that meaning-preserving rewrites retain solvability and solution consistency.
These trends are stable across model sizes and languages, including lower-resource settings.
Together, these results confirm that both perturbation methods produce mathematically valid and solvable questions.
NumEdit reliably changes the target answer, while Paraphrase preserves it, validating their use as controlled probes for disentangling memorization from latent reasoning.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l l r r r r r r r r r r r}
\toprule
Original Model & Metric & EN & FR & DE & ZH & JA & RU & ES & SW & BN & TE & TH \\
\midrule
\multirow{3}{*}{R1-Qwen-7B} & \textbf{Orig Acc} $\uparrow$ & 0.98 & 0.93 & 0.95 & 0.94 & 0.88 & 1.00 & 0.96 & 0.94 & 0.93 & 0.91 & 0.96 \\
 & \textbf{NumEdit Match} $\downarrow$ & 0.07 & 0.05 & 0.08 & 0.06 & 0.16 & 0.07 & 0.07 & 0.16 & 0.05 & 0.08 & 0.09 \\
 & \textbf{Paraphrase Match} $\uparrow$ & 0.97 & 0.93 & 0.99 & 0.95 & 0.97 & 1.00 & 0.95 & 0.97 & 0.93 & 0.87 & 0.91 \\
 \hline
\addlinespace[3pt]
\multirow{3}{*}{R1-Qwen-14B} & \textbf{Orig Acc} $\uparrow$ & 0.97 & 0.96 & 0.94 & 0.94 & 0.88 & 0.95 & 0.94 & 0.86 & 0.99 & 0.89 & 0.96 \\
 & \textbf{NumEdit Match} $\downarrow$ & 0.07 & 0.06 & 0.07 & 0.09 & 0.16 & 0.08 & 0.12 & 0.06 & 0.07 & 0.04 & 0.08 \\
 & \textbf{Paraphrase Match} $\uparrow$ & 0.97 & 0.94 & 0.97 & 0.96 & 0.93 & 0.95 & 0.97 & 0.88 & 0.97 & 0.93 & 0.94 \\
 \hline
\addlinespace[3pt]
\multirow{3}{*}{R1-Qwen-32B} & \textbf{Orig Acc} $\uparrow$ & 0.98 & 0.97 & 0.93 & 0.93 & 0.94 & 0.98 & 0.97 & 0.95 & 0.96 & 0.89 & 0.96 \\
 & \textbf{NumEdit Match} $\downarrow$ & 0.10 & 0.06 & 0.09 & 0.11 & 0.15 & 0.11 & 0.08 & 0.09 & 0.11 & 0.13 & 0.09 \\
 & \textbf{Paraphrase Match} $\uparrow$ & 0.94 & 0.95 & 0.97 & 0.98 & 0.95 & 0.99 & 0.97 & 0.95 & 0.97 & 0.95 & 0.95 \\
\bottomrule
\end{tabular}
}
\caption{Gemini performance on original and counterfactual MGSM questions. \textbf{Orig Acc} compares Gemini's prediction on the original question to the gold answer. \textbf{NumEdit Match} measures the fraction of NumEdit predictions identical to the original prediction (lower is better). \textbf{Paraphrase Match} measures the fraction of Paraphrase predictions identical to the original prediction (higher is better).}
\label{tab:gemini_counterfactuals}
\end{table*}


\begin{figure*}[t]
\centering
\begin{tcolorbox}[
  enhanced,
  colback=white,
  colframe=black!50,
  boxrule=0.6pt,
  arc=2mm,
  left=3mm,right=3mm,top=2mm,bottom=2mm,
  width=\textwidth,
  title=\textbf{Paraphrase prompt template},
  fonttitle=\normalsize,
]
\small
\ttfamily
You are rewriting a math problem.

Language constraint (MUST follow):\\
- The paraphrase MUST be written in the SAME language as the original question.\\
- The original question language is: \{language\_name\}. Do NOT translate to any other language.
\\
Hard constraints:\\
1) Preserve ALL numbers exactly (character-for-character).\\
2) Preserve ALL LaTeX math exactly as-is (anything inside \$...\$ must appear unchanged).\\
3) Keep the question asking for the same final quantity; the problem must be logically equivalent.\\
4) Reduce lexical overlap by paraphrasing and reordering sentences outside math mode.\\
5) Do NOT include any solution steps, explanations, or the final answer.\\
6) Do NOT add or remove any facts, entities, units, or constraints.\\

Return ONLY valid JSON with exactly these keys:\\
\{``paraphrase'': ``...'', ``changes'': ``...''\}

Original problem:
\\
\{problem\}
\\
\end{tcolorbox}
\caption{Prompt used to generate meaning-preserving paraphrases using \texttt{Gemini-2.5-Flash}. Placeholders \{\texttt{language\_name}\} and \{\texttt{problem}\} are substituted per instance.}
\label{fig:paraphrase_prompt}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{tcolorbox}[
  enhanced,
  colback=white,
  colframe=black!50,
  boxrule=0.6pt,
  arc=2mm,
  left=3mm,right=3mm,top=2mm,bottom=2mm,
  width=\textwidth,
  title=\textbf{Solvability evaluation prompt},
  fonttitle=\normalsize,
]
\small
\ttfamily
You are given a grade-school math word problem.\\

Language constraint:\\
- Write your solution in the SAME language as the problem.\\
- The problem language is: \{language\_name\}. Do not translate.\\

You may write intermediate steps.\\
Hard requirement:\\
- End your response with a SINGLE final line in the following exact format:\\
\quad FINAL\_ANSWER: <answer>\\

Rules for <answer>:\\
- Provide only the final numeric value (or a simplified number).\\
- Do not wrap it in LaTeX, do not add units, and do not add extra words.\\
- Do not output anything after the FINAL\_ANSWER line.\\

Problem:
\\
\{problem\}
\\
\end{tcolorbox}
\caption{Prompt used to evaluate the solvability of original and counterfactual MGSM questions using \texttt{Gemini-2.5-Flash}. Placeholders \{\texttt{language\_name}\} and \{\texttt{problem}\} are substituted per instance.}
\label{fig:gemini_solvability_prompt}
\end{figure*}

==> latex/similarity_results.tex <==
\section{Complete Similarity results}\seclabel{similarity_results}

\begin{figure*}
    \centering
    % \setlength{\abovecaptionskip}{-0.05cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/all_langs_en_avg_steps.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/all_langs_en_avg_steps.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/all_langs_en_avg_steps.pdf}
    \caption{Aggregated cosine similarity on \textbf{MGSM} between hidden states in each language and English (reference), averaged over both reasoning steps and layers. 
    High-resource languages show consistently higher similarity to English, suggesting convergence toward an English-centered latent reasoning pathway.}
    \label{fig:cosine_sim_aggregated_mgsm}
\end{figure*}

\begin{figure*}
    \centering
    % \setlength{\abovecaptionskip}{-0.05cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/all_langs_en_avg_layers.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/all_langs_en_avg_steps.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/all_langs_en_avg_steps.pdf}
    \includegraphics[width=0.32\textwidth]{./figures_appendix/cosine_similarities_plot_aggregated_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/all_langs_en_avg_steps.pdf}
    \caption{Aggregated cosine similarity on \textbf{Multilingual AIME} between hidden states in each language and English (reference), averaged over both reasoning steps and layers. 
    High-resource languages show consistently higher similarity to English, suggesting convergence toward an English-centered latent reasoning pathway.}
    \label{fig:cosine_sim_aggregated_aime}
\end{figure*}

\subsection{Similarity with English}\seclabel{sim_eng}

We conduct a focused analysis of crosslingual representational alignment by computing the cosine similarity between hidden states in each target language and those of English.
For each instance, and at each truncation ratio, we extract the hidden state corresponding to the final token of the partial reasoning trace and compare it with the hidden state obtained from the English version of the same problem.
To summarize these similarities, we aggregate them both across layers and across reasoning steps.
Figure~\ref{fig:cosine_sim_aggregated_mgsm} and Figure~\ref{fig:cosine_sim_aggregated_aime} present the resulting trends for MGSM and Multilingual AIME, respectively.

Across both benchmarks, we observe systematic differences in representational alignment with English that seem to correlate with language resource levels: high-resource languages exhibit consistently stronger alignment with English representations, whereas mid- and low-resource languages show reduced alignment.

\subsection{Similarity vs. Correctness}\seclabel{sim_correct}

\begin{figure*}
    \centering

    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/bn_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/bn_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/de_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/de_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/es_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/es_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/fr_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/fr_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ja_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ja_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ru_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ru_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/sw_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/sw_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/te_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/te_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/th_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/th_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/zh_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/zh_en_vs_avgothers_avg_steps.pdf}
    \caption{Comparison of cosine similarity with English versus average similarity with other languages, shown separately for correctly and incorrectly solved examples in \textbf{MGSM} with \textbf{R1-Qwen-7B}.}
    \label{fig:cosine_sim_vs_others_complete_7b}
\end{figure*}

\begin{figure*}
    \centering

    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/bn_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/bn_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/de_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/de_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/es_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/es_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/fr_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/fr_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ja_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ja_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ru_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ru_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/sw_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/sw_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/te_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/te_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/th_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/th_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/zh_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/zh_en_vs_avgothers_avg_steps.pdf}
    \caption{Comparison of cosine similarity with English versus average similarity with other languages, shown separately for correctly and incorrectly solved examples in \textbf{MGSM} with \textbf{R1-Qwen-14B}.}
    \label{fig:cosine_sim_vs_others_complete_14b}
\end{figure*}

\begin{figure*}
    \centering

    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/bn_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/bn_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/de_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/de_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/es_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/es_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/fr_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/fr_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ja_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ja_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ru_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ru_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/sw_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/sw_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/te_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/te_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/th_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/th_en_vs_avgothers_avg_steps.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/zh_en_vs_avgothers_avg_layers.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/cosine_similarities_plots_en_vs_avgothers_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/zh_en_vs_avgothers_avg_steps.pdf}
    \caption{Comparison of cosine similarity with English versus average similarity with other languages, shown separately for correctly and incorrectly solved examples in \textbf{MGSM} with \textbf{R1-Qwen-32B}.}
    \label{fig:cosine_sim_vs_others_complete_32b}
\end{figure*}

We examine whether answer correctness affects crosslingual alignment by grouping MGSM examples into \emph{correct} and \emph{incorrect} sets and comparing their similarity to English and to other languages.
Results for R1-Qwen-\{7B,14B,32B\} are shown in Figures~\ref{fig:cosine_sim_vs_others_complete_7b}, \ref{fig:cosine_sim_vs_others_complete_14b}, \ref{fig:cosine_sim_vs_others_complete_32b}.
Across models, alignment with English seems to vary systematically with language resource level.
High-resource languages show consistently strong similarity to English regardless of correctness, whereas low-resource languages (e.g., Swahili) are more similar to other non-English languages, suggesting a more autonomous latent subspace.
Mid-resource languages exhibit an intermediate pattern, with stronger English alignment primarily for correctly solved instances.


==> latex/truncation_results.tex <==
\section{Complete Truncation Results}\seclabel{truncation_results}

\subsection{Truncation Curves}

Figures~\ref{fig:truncation_7b_mgsm}, \ref{fig:truncation_14b_mgsm}, \ref{fig:truncation_32b_mgsm} and their Multilingual AIME counterparts (Figure~\ref{fig:truncation_7b_aime}, \ref{fig:truncation_14b_aime}, \ref{fig:truncation_32b_aime}) visualize pass@$k$ accuracy ($k=1,5,10$) and the gold-in-trace rate as a function of reasoning-trace truncation ratio across languages and model sizes.
Across models, MGSM exhibits a characteristic pattern in which accuracy increases well before the gold answer is explicitly articulated, whereas on Multilingual AIME accuracy typically remains low until late truncation ratios.
The figures also highlight substantial crosslingual variation, with high-resource languages generally achieving earlier and more stable gains than mid- and low-resource languages.


\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/bn/mgsm_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/de/mgsm_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/en/mgsm_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/es/mgsm_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/fr/mgsm_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ja/mgsm_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ru/mgsm_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/sw/mgsm_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/te/mgsm_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/th/mgsm_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/zh/mgsm_zh_hack_forward.pdf}
    \caption{
    Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-7B} on \textbf{MGSM}. The model shows stronger latent reasoning in high-resource languages (e.g., English).
    }
    \label{fig:truncation_7b_mgsm}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/bn/mgsm_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/de/mgsm_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/en/mgsm_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/es/mgsm_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/fr/mgsm_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ja/mgsm_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ru/mgsm_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/sw/mgsm_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/te/mgsm_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/th/mgsm_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/zh/mgsm_zh_hack_forward.pdf}
    \caption{Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-14B} on \textbf{MGSM}. The model shows stronger latent reasoning in high-resource languages (e.g., English).}
    \label{fig:truncation_14b_mgsm}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/bn/mgsm_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/de/mgsm_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/en/mgsm_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/es/mgsm_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/fr/mgsm_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ja/mgsm_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ru/mgsm_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/sw/mgsm_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/te/mgsm_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/th/mgsm_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/zh/mgsm_zh_hack_forward.pdf}
    \caption{Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-32B} on \textbf{MGSM}. The model shows stronger latent reasoning in high-resource languages (e.g., English).}
    \label{fig:truncation_32b_mgsm}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/bn/aime_multilingual_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/de/aime_multilingual_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/en/aime_multilingual_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/es/aime_multilingual_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/fr/aime_multilingual_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/ja/aime_multilingual_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/ru/aime_multilingual_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/sw/aime_multilingual_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/te/aime_multilingual_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/th/aime_multilingual_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/zh/aime_multilingual_zh_hack_forward.pdf}
    \caption{
    Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-7B} on \textbf{Multilingual AIME}. Latent reasoning is less pronounced compared to MGSM.
    }
    \label{fig:truncation_7b_aime}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/bn/aime_multilingual_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/de/aime_multilingual_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/en/aime_multilingual_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/es/aime_multilingual_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/fr/aime_multilingual_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/ja/aime_multilingual_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/ru/aime_multilingual_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/sw/aime_multilingual_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/te/aime_multilingual_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/th/aime_multilingual_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/zh/aime_multilingual_zh_hack_forward.pdf}
    \caption{
    Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-14B} on \textbf{Multilingual AIME}. Latent reasoning is less pronounced compared to MGSM.
    }
    \label{fig:truncation_14b_aime}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/bn/aime_multilingual_bn_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/de/aime_multilingual_de_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/en/aime_multilingual_en_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/es/aime_multilingual_es_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/fr/aime_multilingual_fr_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/ja/aime_multilingual_ja_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/ru/aime_multilingual_ru_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/sw/aime_multilingual_sw_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/te/aime_multilingual_te_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/th/aime_multilingual_th_hack_forward.pdf}
    \includegraphics[width=0.23\textwidth]{./figures_appendix/plots_trunc_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/zh/aime_multilingual_zh_hack_forward.pdf}
    \caption{
    Pass@$k$ accuracy ($k=1,5,10$) and gold-in-trace rate under reasoning-trace truncation for \textbf{R1-Qwen-32B} on \textbf{Multilingual AIME}. Latent reasoning is less pronounced compared to MGSM.
    }
    \label{fig:truncation_32b_aime}
\end{figure*}

\subsection{Causal Decompositions}

Figures~\ref{fig:interval_7b_mgsm}, \ref{fig:interval_14b_mgsm}, \ref{fig:interval_32b_mgsm} (MGSM) and Figures~\ref{fig:interval_7b_aime}, \ref{fig:interval_14b_aime}, \ref{fig:interval_32b_aime} (Multilingual AIME) further decompose accuracy gains between consecutive truncation intervals into three cases:
(i) the gold answer is newly articulated in the added reasoning steps,
(ii) it was already present earlier in the visible trace, or
(iii) it has not yet appeared in the truncated trace.
This analysis disentangles improvements driven by explicit answer articulation from those arising prior to any verbalized solution.
On MGSM, gains at early and intermediate truncation ratios are largely attributed to case (iii), indicating that correct predictions often emerge before the answer is explicitly articulated.
In contrast, on Multilingual AIME, gains are sparser and increasingly dominated by cases (i) and (ii), reflecting a stronger dependence on explicit reasoning and a reduced role for early latent solution formation.



\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-7B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{MGSM} with \textbf{R1-Qwen-7B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Early and intermediate gains are dominated by case (\textbf{iii}), indicating latent reasoning.
    }
    \label{fig:interval_7b_mgsm}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-14B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{MGSM} with \textbf{R1-Qwen-14B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Early and intermediate gains are dominated by case (\textbf{iii}), indicating latent reasoning.
    }
    \label{fig:interval_14b_mgsm}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/mgsm/DeepSeek-R1-Distill-Qwen-32B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{MGSM} with \textbf{R1-Qwen-32B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Early and intermediate gains are dominated by case (\textbf{iii}), indicating latent reasoning.
    }
    \label{fig:interval_32b_mgsm}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-7B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{Multilingual AIME} with \textbf{R1-Qwen-7B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Compared to MGSM, gains are sparser and less dominated by latent reasoning.
    }
    \label{fig:interval_7b_aime}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-14B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{Multilingual AIME} with \textbf{R1-Qwen-14B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Compared to MGSM, gains are sparser and less dominated by latent reasoning.
    }
    \label{fig:interval_14b_aime}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/bn/bn_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/de/de_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/en/en_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/es/es_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/fr/fr_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/ja/ja_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/ru/ru_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/sw/sw_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/te/te_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/th/th_hack_forward_passat1_causality_bars.pdf}
    \includegraphics[width=0.24\textwidth]{./figures_appendix/plots_trunc_causal_bars_merged/aime_multilingual/DeepSeek-R1-Distill-Qwen-32B/zh/zh_hack_forward_passat1_causality_bars.pdf}
    \caption{
    Causal decomposition of newly correct predictions across truncation intervals on \textbf{Multilingual AIME} with \textbf{R1-Qwen-32B}.
    Each bar partitions gains into three cases: (\textbf{i}) the gold answer is first articulated in the newly added reasoning steps,
    (\textbf{ii}) it was already articulated in earlier steps, or
    (\textbf{iii}) it has not yet appeared in the visible truncated trace.
    Compared to MGSM, gains are sparser and less dominated by latent reasoning.
    }
    \label{fig:interval_32b_aime}
\end{figure*}

